A Tale of Two Cities: Software Developers Working from Home During the COVID-19 Pandemic

The COVID-19 pandemic has shaken the world to its core and has provoked an overnight exodus of developers that normally worked in an office setting to working from home. The magnitude of this shift and the factors that have accompanied this new unplanned work setting go beyond what the software engineering community has previously understood to be remote work. To find out how developers and their productivity were affected, we distributed two surveys (with a combined total of 3,634 responses that answered all required questions) -- weeks apart to understand the presence and prevalence of the benefits, challenges, and opportunities to improve this special circumstance of remote work. From our thematic qualitative analysis and statistical quantitative analysis, we find that there is a dichotomy of developer experiences influenced by many different factors (that for some are a benefit, while for others a challenge). For example, a benefit for some was being close to family members but for others having family members share their working space and interrupting their focus, was a challenge. Our surveys led to powerful narratives from respondents and revealed the scale at which these experiences exist to provide insights as to how the future of (pandemic) remote work can evolve.

==> tables/relatedwork-methods.tex <==
\begin{landscape}
\begin{table}
%
\centering
\caption{Comparing the research goals, research methods, key findings and implications from the studies that have studied developers as they work from home during the COVID-19 pandemic.}
\label{tab:relatedwork}
\renewcommand{\arraystretch}{1.5} 
\newlength{\relTableColumnA}
\newlength{\relTableColumnB}
\newlength{\relTableColumnC}
\newlength{\relTableColumnD}
\newlength{\relTableColumnE}
\settowidth{\relTableColumnA}{Research questions/XX}
\settowidth{\relTableColumnB}{(longer days/more weekends)}
\settowidth{\relTableColumnC}{- Change in wellbeing depends on}
\settowidth{\relTableColumnD}{- Main benefits of WFH: no commute,}
\settowidth{\relTableColumnE}{- Main benefits of WFH: no commute,}
\scalebox{0.8}{
\begin{tabular}{|p{\relTableColumnA}|p{\relTableColumnB}|p{\relTableColumnC}|p{\relTableColumnD}|p{\relTableColumnE}|}
\hline
& \textbf{GitHub COVID-19 Study \newline (Forsgren et al., 2020)~\cite{forsgren2020covid}}
& \textbf{Pandemic Programming \newline (Ralph et al., 2020)~\cite{ralph2020pandemic}}
& \textbf{Baidu COVID-19 Study \newline (Bao et al., 2020)~\cite{bao2020does}}
& \textbf{Microsoft study \newline (This paper)}
\\ \hline
\textbf{Research questions/\newline goals}
& \raggedright Understand dev productivity, work cadence, collaboration during early COVID-19
& \raggedright Understand how WFH due to COVID-19 affects dev wellbeing and productivity
& \raggedright Understand impact of WFH on productivity
& {\raggedright Understand benefits/challenges since WFH and factors that affect productivity over time}
\\ \hline
\textbf{Research methods}
& \raggedright Descriptive analysis of GitHub developer activity
& \raggedright Survey to test hypotheses of dev experience since WFH
& \raggedright Analysis of dev activity records and survey
& {\raggedright Surveys (exploratory, quantitative)} %
\\ \hline
\textbf{Population}
& \raggedright Open source projects and paid/enterprise accounts
& \raggedright Software developers anywhere in the world
& \raggedright Baidu developers in China
& {\raggedright Microsoft engineers (devs and program managers in Puget Sound (\surveyone) and US (\surveytwo)} %
\\ \hline
\textbf{Participants/data}
& \raggedright Data from all open source/ paid accounts
& \raggedright Approx. 2.25K survey responses from 53 countries (23\% Germany, 16\% Russia, 12\% Italy, 4\% USA)
& \raggedright 139 devs' activities over 138 days
& {\raggedright \surveyoneresponses responses (\surveyone) \newline \surveytworesponses responses (\surveytwo)} %
\\ \hline
\textbf{Timing}
& \raggedright Jan - March, 2020 (compared with Jan-March 2019)
& \raggedright March 19-April 14, 2020
& \raggedright Dec 2019 to March 2020, compared with 2019
& {\raggedright March 16-20, 2020 (\surveyone). \newline April 22-May 9, 2020 (\surveytwo) }
\\ \hline
\textbf{Findings}
& \raggedright - Dev activity consistent or increased since last year\newline - Work cadence changed (longer days/more weekends)\newline - More collaboration (esp in open source) 
& \raggedright - Change in wellbeing and productivity \newline - Change in productivity depends on ergonomics/disaster prep\newline - Change in wellbeing depends on ergonomics and fear\newline - People with children have less ergonomic home offices\newline - People with disabilities less prepared for disasters 
& \raggedright - WFH has different impacts on dev  productivity (varies by project age/type/language/size/metric)\newline - Productivity of majority of devs when WFH is similar to onsite\newline - For those that are more productive, they feel more enthusiastic/focused and have better work life balance\newline - For those less productive they have more home chores, harder collab 
& {\raggedright - Main challenges of WFH: miss social interactions, poor work life boundary, poor ergonomics, less awareness of others' work, less exercise, difficult communication, for some lack of childcare\newline - Main benefits of WFH: no commute, money, flexible hours, close to family, comfort at home, health, time\newline - Identify the main challenges and benefits that explain both positive and negative changes in productivity}  
\\ \hline
\textbf{Implications/\newline recommendations} 
& \raggedright - Plan tool/process flexibility\newline - Embrace collaboration\newline - Anticipate burnout
& \raggedright - Pay for home internet charges\newline - Care about employee wellbeing\newline - Little consensus among devs what orgs can do to help
& \raggedright - WFH should be a choice\newline - Project characteristics matter\newline - Individual devs need different strategies if WFH
& {\raggedright - Dichotomous experiences for same factors, support all/part WFH options\newline - Provide better hardware, internet, stipend, software, guidelines, support}
\\ \hline
\end{tabular}
}
%
\end{table}
\end{landscape}

